NExG: Provable and Guided State Space Exploration of Neural Network Control Systems using Sensitivity Approximation

We propose a new technique for performing state space exploration of closed loop control systems with neural network feedback controllers. Our approach involves approximating the sensitivity of the trajectories of the closed loop dynamics. Using such an approximator and the system simulator, we present a guided state space exploration method that can generate trajectories visiting the neighborhood of a target state at a specified time. We present a theoretical framework which establishes that our method will produce a sequence of trajectories that will reach a suitable neighborhood of the target state. We provide thorough evaluation of our approach on various systems with neural network feedback controllers of different configurations. We outperform earlier state space exploration techniques and achieve significant improvement in both the quality (explainability) and performance (convergence rate). Finally, we adopt our algorithm for the falsification of a class of temporal logic specification, assess its performance against a state-of-the-art falsification tool, and show its potential in supplementing existing falsification algorithms.

==> psd-macros.tex <==
\usepackage{tikz}
\usepackage[usenames,dvipsnames]{pstricks}
%\usepackage{epsfig} -- here

%\usepackage{palatino}
\RequirePackage{ifthen}
% \RequirePackage{amsmath}
% \RequirePackage{amssymb}
\RequirePackage{listings}
\RequirePackage{mathrsfs}
\RequirePackage{xspace}
\RequirePackage{graphics}

% PACKAGES FOR ORGANIZING THE STRUCTE OF DOCUMENT
%\usepackage{minipage}
\usepackage{latexsym}
\usepackage{multicol}
\usepackage{multirow}
\usepackage{lscape}  % Useful for wide tables or figures.
\usepackage{xspace}
\usepackage{paralist}
%\usepackage{framed}
%\usepackage{lipsum}
% DEFINING THE BOUNDARY --- DONE IN DOCUMENT.
%\usepackage[left=1.25in,right=1.25in,top=1in,bottom=1.25in]{geometry}

%%% SECTION TITLE APPEARANCE
% \usepackage{sectsty}
% \allsectionsfont{\sffamily\mdseries\upshape} % (See the fntguide.pdf for font help)
% (This matches ConTeXt defaults)

%%% HEADERS & FOOTERS
% \usepackage{fancyhdr} % This should be set AFTER setting up the page geometry
% \pagestyle{fancy} % options: empty , plain , fancy
% \renewcommand{\headrulewidth}{0pt} % customise the layout...
% \lhead{}\chead{}\rhead{}
% \lfoot{}\cfoot{\thepage}\rfoot{}


% PACKAGES FOR FIGURES
\usepackage{xcolor}
\usepackage{float}
%\usepackage{subfigure} -- here
\usepackage{subfloat}
\usepackage{graphicx}
\usepackage{caption}
\usepackage{wrapfig}
%\usepackage{pifont}
%\usepackage{subcaption}
%\usepackage{subfigure}  % for subfigures
%\usepackage{setspace}
%\usepackage[justification=raggedright]{caption}	% makes captions ragged right - thanks to Bryce Lobdell

%AMS AND OTHER MISC PACKAGES
\usepackage{keyval}
\usepackage{amsmath,amssymb,amsfonts,url,listings,mathrsfs}
%reference
%\usepackage[pdftex,colorlinks,citecolor=webblue,linkcolor=webblue,urlcolor=webblue]{hyperref} -- here

%ALGORITHM PACKAGE
%\usepackage{algorithm,algorithmic}
%
%\usepackage[pdftex,colorlinks,citecolor=webblue,linkcolor=webred,backref,pagebackref]{hyperref}
%\usepackage[linesnumbered,lined,commentsnumbered]{algorithm2e}
%\usepackage[linesnumbered,boxed,lined,commentsnumbered,algochapter]{algorithm2e}


%DEFINITIONS FOR MARKING CHANGES AND COMMENTS
\newcommand{\authcomment}[1]{\textbf{[[#1]]}}
%\newcommand{\sayan}[1]{\textcolor{blue}{[[#1]]}}
%\newcommand{\sridhar}[1]{\textcolor{red}{[[#1]]}}
\newcommand{\sridhar}[1]{\textcolor{brown}{[[#1]]}}

% DEFINING COLORS
\definecolor{reddish}{rgb}{1,.8,0.8}
\definecolor{blueish}{rgb}{0.8,.8,1}
\definecolor{greenish}{rgb}{.8,1,0.8}
\definecolor{yellowish}{rgb}{1,1,.20}
\definecolor{webred}{rgb}{0.5,0,0}
\definecolor{webblue}{rgb}{0,0,0.8}

% DEFINITIONS FOR TEXT FORMATTING
\newcommand{\figuresize}{\scriptsize}
\newcommand{\equationsize}{\footnotesize}

% ADHOC DEFINITIONS FOR EACH AND EVERY PAPER
\newcommand{\trajmet}{discrepancy function\/}
\newcommand{\TrajMet}{Trajectory Metric}
\newcommand{\RT}{{\em reachtubes}}
\newcommand{\valsim}{{\sf valSim}}
\newcommand{\tool}{C2E2 \/}
\newcommand{\fulltoolname}{\textbf{C}heck \textbf{E}xecute \textbf{C}ompare \textbf{E}ngine}
\newcommand{\leftshift}[2]{\relax\ifmmode (#1 \lhd #2) \else $(#1 \lhd #2)$ \fi}
\newcommand{\mayInt}{\relax\ifmmode \mathit{mayInt} \else $\mathit{mayInt}$ \fi}
\newcommand{\mustInt}{\relax\ifmmode \mathit{mustInt} \else $\mathit{mustInt}$ \fi}
\newcommand{\notInt}{\relax\ifmmode \mathit{notInt} \else $\mathit{notInt}$ \fi}
\newcommand{\alarm}{\relax\ifmmode \mathit{Alert} \else $\mathit{Alert}$ \fi}
\newcommand{\unsafe}{\relax\ifmmode \mathit{Unsafe} \else $\mathit{Unsafe}$ \fi}
\newcommand{\xsep}{\relax\ifmmode \mathit{xsep} \else $\mathit{xsep}$\fi}
\newcommand{\ysep}{\relax\ifmmode \mathit{ysep} \else $\mathit{ysep}$ \fi}
\newcommand{\etime}{{\sf time}}
\newcommand{\ub}{{\sf ub}}
\newcommand{\lb}{{\sf lb}}
\newcommand{\emode}{{\sf mode}}
\newcommand{\erange}{{\sf range}}
\newcommand{\fbls} {functionally bounded linear span}
\newcommand{\fblsupper} {Functionally bounded linear span}

% COMMANDS USED IN DEFINITIONS
\newcommand{\meansl}{[\![}
\newcommand{\meansr}{]\!]}
\newcommand{\means}[1]{\meansl #1 \meansr}
\newcommand{\Nset}[1]{[[#1]]}

% ROUTINELY USED COMMANDS
\newcommand{\refinement}[1]{\relax\ifmmode \mathit{refine}(#1) \else $\mathit{refine}(#1)$ \fi}
\newcommand{\diff}{{\sf diff}}
\newcommand{\diameter} {\mathsf{diameter}}
\newcommand{\cntr} {\mathsf{center}}
\newcommand{\ball}[1] {B_{#1}}
\newcommand{\true}{\relax\ifmmode \mathit true \else \em true \/\fi}
\newcommand{\false}{\relax\ifmmode \mathit false \else \em false \/\fi}
% \newcommand{\lnot}{\neg} % Already defined
% \newcommand{\land}{\wedge} % Already defined
% \newcommand{\lor}{\vee} % Already defined
\newcommand{\limplies}{\Rightarrow}
\newcommand{\liff}{\Leftrightarrow}
%\newcommand{\T}{\mathit{true}}
%\newcommand{\F}{\mathit{false}}
% \newcommand{\to}{\relax\ifmmode \rightarrow \else $\rightarrow$\fi} % Already defined
\newcommand{\fro}{\relax\ifmmode \leftarrow \else $\leftarrow$\fi}


% COMMANDS FOR MATH SPECIFIC ITEMS
\newcommand{\nnt}{{\sf T}^{\geq 0}}             %nonnegative time points
\newcommand{\post}{{\sf T}^{>0}}                %positive time points
\newcommand{\Variables}{{\sf V}}                %variables

\newcommand{\num}[1]{\relax\ifmmode \mathbb #1\else $\mathbb #1$\fi}
\newcommand{\nnnum}[1]{\relax\ifmmode 
  {\mathbb #1}_{\geq 0} \else ${\mathbb #1}_{\geq 0}$
  \fi}
\newcommand{\npnum}[1]{\relax\ifmmode 
  {\mathbb #1}_{\leq 0} \else ${\mathbb #1}_{\leq 0}$
  \fi}
\newcommand{\pnum}[1]{\relax\ifmmode 
  {\mathbb #1}_{> 0} \else ${\mathbb #1}_{> 0}$
  \fi}
\newcommand{\nnum}[1]{\relax\ifmmode 
  {\mathbb #1}_{< 0} \else ${\mathbb #1}_{< 0}$
  \fi}
\newcommand{\plnum}[1]{\relax\ifmmode 
  {\mathbb #1}_{+} \else ${\mathbb #1}_{+}$
  \fi}
\newcommand{\nenum}[1]{\relax\ifmmode 
  {\mathbb #1}_{-} \else ${\mathbb #1}_{-}$
  \fi}

\newcommand{\reals}{{\num R}}                    %reals
\newcommand{\nnreals}{{\nnnum R}}                    %nonnegative reals
\newcommand{\realsinfty}{{\num R} \cup \{\infty, -\infty\}}                    %nonnegative reals
\newcommand{\plreals}{{\plnum R}}                    %positive reals
\newcommand{\naturals}{{\num N}}                      %natural numbers
\newcommand{\integers}{{\num Z}}                      %integers
\newcommand{\rationals}{{\num Q}}                      %rationals
\newcommand{\nnrationals}{{\nnnum Q}}                   % nonnegative rationals
\newcommand{\Time}{{\num T}}  
\newcommand{\bools}{{\num B}}  
\newcommand{\plintegers}{{\plnum Z}}                      %integers
\newcommand{\deq}{\mathrel{\stackrel{\scriptscriptstyle\Delta}{=}}}
\newcommand{\intervals}{\relax \ifmmode \mathbb{IR} \else $\mathbb{IR}$ \fi}
\newcommand{\nnintervals}{\relax \ifmmode \mathbb{IR}^{+} \else $\mathbb{IR}^{+}$ \fi}
%\setlength{\mathindent}{0pt}

% COMMANDS FOR LABELS
\renewcommand{\eqref}[1]{Equation~(\ref{eq:#1})}
\newcommand{\eqlabel}[1]{\label{eq:#1}}
\newcommand{\figref}[1]{Figure~\ref{fig:#1}}
\newcommand{\figrefs}[2]{Figures~\ref{fig:#1} and~\ref{fig:#2}}
\newcommand{\figlabel}[1]{\label{fig:#1}}
\newcommand{\tabref}[1]{Table~\ref{table:#1}}
\newcommand{\tablabel}[1]{\label{table:#1}}
\newcommand{\defref}[1]{Definition~\ref{def:#1}}
\newcommand{\deflabel}[1]{\label{def:#1}}
\newcommand{\exref}[1]{Example~\ref{exmp:#1}}
\newcommand{\exlabel}[1]{\label{exmp:#1}}
\newcommand{\scref}[1]{Section~\ref{sec:#1}}
\newcommand{\secreftwo}[2]{Sections~\ref{sec:#1}~and~\ref{sec:#2}}
\newcommand{\sclabel}[1]{\label{sec:#1}}
\newcommand{\applabel}[1]{\label{app:#1}}
\newcommand{\appref}[1]{Appendix~\ref{app:#1}}
\newcommand{\lnlabel}[1]{\label{line:#1}}
\newcommand{\lnrngref}[2]{lines~\ref{line:#1}--\ref{line:#2}\xspace}
\newcommand{\lnref}[1]{line~\ref{line:#1}\xspace}
\newcommand{\thmref}[1]{Theorem~\ref{thm:#1}\xspace}
%\newcommand{\seclabel}[1]{\label{sec:#1}}
%\newcommand{\secref}[1]{Section~\ref{sec:#1}}
%\newcommand{\figlabel}[1]{\label{fig:#1}}
%\newcommand{\figref}[1]{Figure~\ref{fig:#1}}


% COMMANDS FOR SECTIONS AND ORGANIZATION

\newenvironment{noqedproof}{\pf}{}
\newcommand{\pf}{\par\noindent{\bf Proof:}~}
% \newcounter{theorem}
% \setcounter{theorem}{0}
% 
%  \newtheorem{theorem}{Theorem}
%  \newtheorem{lemma}[theorem]{Lemma}
%  \newtheorem{corollary}[theorem]{Corollary}
%  \newtheorem*{claim}{Claim}
%  \newtheorem{assumption}{Assumption}
%  \theoremstyle{definition}
%  \newtheorem{definition}{Definition}
%  \newcommand{\qed}{\hfill{\rule{2mm}{2mm}}\medskip}
%  \newenvironment{proof}{\pf}{\qed}
%  \newtheorem{proposition}[theorem]{Proposition}
% \newtheorem{inv}[theorem]{Invariant}
 
%    \newcounter{rem}
%  \setcounter{rem}{0}
%  
%   \newenvironment{remark}
%   {\refstepcounter{rem} \vspace{2ex}\par\noindent
%    \textbf{Remark}~\textbf{\therem~}}
 
% \newcounter{example}
%  \setcounter{example}{0}

%   \newtheorem{example}[example]{Example}
%  \newcounter{example}
  
%  \newenvironment{example}
%  {\refstepcounter{example} \vspace{2ex}\par\noindent
%  \textbf{Example}~\textbf{\theexample~}}%{\qed}
% \newexample{example}[example]{Example}

%\theoremstyle{remark}
%\newcounter{example}
% \newtheorem{example}{Example}[chapter]
% {\refstepcounter{theorem} \vspace{2ex}\par\noindent
% \textbf{Example}~\textbf{\theexampletheorem~}}{\qed}
 
 \def\examplenonum#1#2{
        \vspace{.15in}
        \noindent
        {\bf Example #1}{\em ~(continued)}{\bf .}
        {#2}{\qed}
        }
        
% \renewcommand{\theequation}{\thesection.\arabic{equation}}
% \renewcommand{\thefigure}{\thesection.\arabic{figure}}
% \renewcommand{\thetable}{\thesection.\arabic{table}}
% \newcommand{\Section}[1]{\section{#1}%
%    \setcounter{equation}{0}\setcounter{figure}{0}\setcounter{table}{0}%
%    \setcounter{example}{0}}


%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%
%%%%% TIOA STUFF %%%%%
%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%



% EXECUTIONS TRACES and FRAGS
\newcommand{\extb}[1]{\relax\ifmmode {\sf ExtBeh}_{#1} \else ${\sf ExtBeh}_{#1}$\fi} 
\newcommand{\tdists}[1]{\relax\ifmmode {\sf Tdists}_{#1} \else ${\sf Tdists}_{#1}$\fi} 

\newcommand{\exec}[1]{\relax\ifmmode {\sf Execs}_{#1} \else ${\sf Exec}_{#1}$\fi} 
\newcommand{\execf}[1]{\relax\ifmmode {\sf Execs}^*_{#1} \else ${\sf Exec}^*_{#1}$\fi} 
\newcommand{\execi}[1]{\relax\ifmmode {\sf Execs}^\omega_{#1} \else ${\sf Exec}^\omega_{#1}$\fi} 

\newcommand{\ctrace}[1]{\relax\ifmmode {\sf Ctraces}_{#1} \else ${\sf Ctraces}_{#1}$\fi} 

\newcommand{\trace}[1]{\relax\ifmmode {\sf Traces}_{#1} \else ${\sf Traces}_{#1}$\fi} 
\newcommand{\tracef}[1]{\relax\ifmmode {\sf Traces}^*_{#1} \else ${\sf Traces}^*_{#1}$\fi} 
\newcommand{\tracei}[1]{\relax\ifmmode {\sf Traces}^\omega_{#1} \else ${\sf Traces}^\omega_{#1}$\fi} 

\newcommand{\frag}[1]{\relax\ifmmode {\sf Frags}_{#1} \else ${\sf Frags}_{#1}$\fi} 
\newcommand{\fragf}[1]{\relax\ifmmode {\sf Frags}^*_{#1} \else ${\sf Frags}^*_{#1}$\fi} 
\newcommand{\fragi}[1]{\relax\ifmmode {\sf Frags}^\omega_{#1} \else ${\sf Frags}^\omega_{#1}$\fi} 

\newcommand{\reach}[1]{\relax\ifmmode {\sf Reach}_{#1} \else ${\sf Reach}_{#1}$\fi} 
\newcommand{\pair}[2]{\relax\ifmmode \langle #1, #2 \rangle \else $\langle #1, #2 \rangle$\fi} 

\newcommand{\TE}{\relax\ifmmode \mathit{Time} \else $\mathit{Time}$ \fi} 
\newcommand{\EQ}{\relax\ifmmode \mathit{Enq} \else $\mathit{Enq}$ \fi} 
\newcommand{\DQ}{\relax\ifmmode \mathit{Deq} \else $\mathit{DeqTime}$ \fi} 
\newcommand{\E}{\relax\ifmmode \mathsf{E} \else $\mathsf{E}$ \fi}

\newcommand{\loc}{\relax\ifmmode \mathit{loc} \else $\mathit{loc}$ \fi}
\newcommand{\abs}{\relax\ifmmode \mathit{abs} \else $\mathit{abs}$ \fi}

\newcommand{\execs}{{\exec{}}}
\newcommand{\traces}{{\trace{}}}
\newcommand{\fragss}{{\frag{}}}
\newcommand{\fexecs}{{\execf{}}}
\newcommand{\ftraces}{{\tracef{}}}
\newcommand{\ffragss}{{\fragf{}}}
\newcommand{\iexecs}{{\execi{}}}
\newcommand{\itraces}{{\tracei{}}}
\newcommand{\ifragss}{{\fragi{}}}
\newcommand{\fstate}{{\sf fstate}}  
\newcommand{\lstate}{{\sf lstate}}  
\newcommand{\ltime}{{\sf ltime}}  
\newcommand{\dur}{{\sf dur}}  
\newcommand{\mode}{{\sf mode}}  
\newcommand{\ftime}{{\sf ftime}}  

% 
% \newenvironment{anotation}[1][Nancy]{\begin{quote}\small[[[#1]]]}{\normalsize\end{quote}}
% \newcommand{\ba}{\begin{anotation}}
% \newcommand{\ea}{\end{anotation}}
% 
% \newcommand{\bcb}{\chgbarbegin}
% \newcommand{\ecb}{\chgbarend}
% \chgbarwidth 1pt
% 
% \newcommand{\dec}{\ensuremath{{:}}}
% \newcommand{\eqdef}{\mathbin{::=}}
% \newcommand{\I}{{\ensuremath{\cap}}}



% OPERATIONS ON SETS, RELATIONS AND FUNCTIONS
\newcommand{\pow}[1]{{\bf P}(#1)} % powerset
\newcommand{\inverse}[1]{#1^{-1}}
\newcommand{\range}[1]{\ms{range{(#1)}}}
\newcommand{\domain}[1]{{\it dom}(#1)}
\newcommand{\type}[1]{\ms{type{(#1)}}}
\newcommand{\dtype}[1]{\ms{dtype{(#1)}}} % dynamic type
\newcommand{\restr}{\mathrel{\lceil}}
\newcommand{\proj}{\matrel{\lceil}}
\newcommand{\restrrange}{\mathrel{\downarrow}}
\newcommand{\point}[1]{\wp(#1)}                 %point trajectory



% HYBRID AUTOMATA
\def\A{{\cal A}} % HA
\def\B{{\cal B}} % HA
\def\C{{\cal C}} % HA
\def\D{{\cal D}} % set of discrete steps
\def\E{{\cal E}} % HA
\def\F{{\cal F}} % HA
\def\G{{\cal G}} % pieces of SHIOA
\def\H{{\cal H}} % HA
\def\I{{\cal I}} % environment sequence
\def\K{{\cal K}} % environment sequence
\def\L{{\cal L}} % environment sequence
\def\M{{\cal M}} % Mode switching transitions
\def\O{{\cal O}} % outcome function
\def\P{{\cal P}} % set of modes
\def\Q{{\cal Q}} % set of modes
\def\R{{\cal R}} % relation
\def\S{{\cal S}} % set of trajectories
\def\T{{\cal T}} % set of trajectories
\def\V{{\cal V}} % Lyapunov function
\def\U{{\cal U}} % set of trajectories
\def\X{{\cal X}} % Lyapunov function
\def\Y{{\cal Y}} % set of trajectories
\def\Z{{\cal Z}} % set of trajectories

\def\u{{\mathsf u}} % set of inputs

% more special characters

\newcommand{\col}[1]{\relax\ifmmode \mathscr #1\else $\mathscr #1$\fi}
\def\statemodels{\col{S}}


% Names of actions, automata etc
\definecolor{HIOAcolor}{rgb}{0.776,0.22,0.07}
\newcommand{\HIOA}{\textcolor{HIOAcolor}{\tt HIOA\hspace{3pt}}}
\newcommand{\PVS}{\textcolor{HIOAcolor}{\tt PVS\hspace{3pt}}}
\newcommand{\PVSnogap}{\textcolor{HIOAcolor}{\tt PVS\hspace{1pt}}}
\newcommand{\HIOAbiggap}{\textcolor{HIOAcolor}{\tt HIOA\hspace{6pt}}}
\newcommand{\HIOAnogap}{\textcolor{HIOAcolor}{\tt HIOA}}
\newcommand{\anyrelation}{\lessgtr}

% Transformation for ADT
\newcommand{\SC}[2]{\relax\ifmmode {\tt Scount}(#1,#2) \else ${\tt Scount}(#1,#2)$\fi} 
\newcommand{\SCM}[2]{\relax\ifmmode {\tt Smin}(#1,#2) \else ${\tt Smin}(#1,#2)$\fi} 
\newcommand{\Aut}[1]{\relax\ifmmode {\tt Aut}(#1) \else ${\tt Aut}(#1)$\fi} 

\newcommand{\auto}[1]{{\operatorname{\mathsf{#1}}}}
\newcommand{\act}[1]{{\operatorname{\mathsf{#1}}}}
\newcommand{\smodel}[1]{{\operatorname{\mathsf{#1}}}}
\newcommand{\pvstheory}[1]{{\operatorname{\mathit{#1}}}}
%\newcommand{\auto}[1]{\relax\ifmmode \sf #1\else $\sf #1$\fi}
%\newcommand{\act}[1]{\relax\ifmmode \sf #1\else $\sf #1$\fi}


\newcommand{\Automaton}{{\bf automaton}}
\newcommand{\Asserts}{{\bf asserts}}
\newcommand{\Assumes}{{\bf assumes}}
\newcommand{\Backward}{{\bf backward}}
\newcommand{\By}{{\bf by}}
%\newcommand{\Case}{{\bf case}} -- here
\newcommand{\Choose}{{\bf  choose}}
\newcommand{\Components}{{\bf components}}
\newcommand{\Const}{{\bf const}}
\newcommand{\Converts}{{\bf converts}}
\newcommand{\Do}{{\bf do}}
\newcommand{\Eff}{{\bf eff}}
%\newcommand{\Else}{{\bf else}} -- here
\newcommand{\Elseif}{{\bf elseif}}
\newcommand{\Enumeration}{{\bf enumeration}}
\newcommand{\Ensuring}{{\bf ensuring}}
\newcommand{\Exempting}{{\bf exempting}}
\newcommand{\Fi}{{\bf fi}}
%\newcommand{\For}{{\bf for}} -- here
\newcommand{\Forward}{{\bf forward}}
\newcommand{\Freely}{{\bf freely}}
\newcommand{\From}{{\bf from}}
\newcommand{\Generated}{{\bf generated}}
\newcommand{\Local}{{\bf local}}
\newcommand{\Hidden}{{\bf hidden}}
%\newcommand{\If}{{\bf if}}  -- here
\newcommand{\In}{{\bf in}}
\newcommand{\Implies}{{\bf implies}}
\newcommand{\Includes}{{\bf includes}}
\newcommand{\Introduces}{{\bf introduces}}
\newcommand{\Input}{{\bf input}}
\newcommand{\Kind}{{\bf kind}}
\newcommand{\Initially}{{\bf initially}}
\newcommand{\Internal}{{\bf internal}}
\newcommand{\Invariant}{{\bf invariant}}
\newcommand{\Od}{{\bf od}}
\newcommand{\Of}{{\bf of}}
\newcommand{\Output}{{\bf output}}
\newcommand{\Partitioned}{{\bf partitioned}}
\newcommand{\Pre}{{\bf pre}}
\newcommand{\Signature}{{\bf signature}}
\newcommand{\Simulation}{{\bf simulation}}
\newcommand{\Sort}{{\bf sort}}
\newcommand{\States}{{\bf states}}
\newcommand{\Tasks}{{\bf tasks}}
\newcommand{\Then}{{\bf then}}
\newcommand{\To}{{\bf to}}
\newcommand{\Trait}{{\bf trait}}
\newcommand{\Traits}{{\bf traits}}
\newcommand{\Transitions}{{\bf transitions}}
\newcommand{\Tuple}{{\bf tuple}}
\newcommand{\Type}{{\bf type}}
\newcommand{\Union}{{\bf union}}
\newcommand{\Uses}{{\bf uses}}
\newcommand{\Where}{{\bf where}}
%\newcommand{\While}{{\bf while}} -- here
\newcommand{\With}{{\bf with}}

% Spacing
\newcommand{\FFF}{\vspace{0.1in}}
\newcommand{\BBB}{\hspace{-0.1in}}


